Progressive Semantic Segmentation

The objective of this work is to segment high-resolution images without overloading GPU memory usage or losing the fine details in the output segmentation map. The memory constraint means that we must either downsample the big image or divide the image into local patches for separate processing. However, the former approach would lose the fine details, while the latter can be ambiguous due to the lack of a global picture. In this work, we present MagNet, a multi-scale framework that resolves local ambiguity by looking at the image at multiple magnification levels. MagNet has multiple processing stages, where each stage corresponds to a magnification level, and the output of one stage is fed into the next stage for coarse-to-fine information propagation. Each stage analyzes the image at a higher resolution than the previous stage, recovering the previously lost details due to the lossy downsampling step, and the segmentation output is progressively refined through the processing stages. Experiments on three high-resolution datasets of urban views, aerial scenes, and medical images show that MagNet consistently outperforms the state-of-the-art methods by a significant margin.

==> experiments_old.tex <==
\textcolor{red}{Chuong is editing}

We evaluate the performance of our MagNet framework on three high resolution datasets: Cityscapes \cite{Cordts2016Cityscapes}, DeepGlobe \cite{demir2018deepglobe}, and Gleason \cite{gleason2019}. The information of these datasets are described in \Tref{tab:datasets}. The number of pixels of each image is from 2 millions to 25 millions. In this section, we present experiments comparing our method with other state-of-the-art methods in semantic segmentation refinement and also describe some ablation studies on Cityscapes dataset.

\begin{table}[t]
    \centering
    \caption{{\bf Details of high-resolution datasets used to evaluate our framework.} All images has from 2 to 25 million pixels with a lot of details.}
    \label{tab:datasets}
    \begin{tabu} to \columnwidth {@{}X[3,l]X[3,c]X[2,c]X[2,c]@{}}
    \toprule
    Dataset & Content & Resolution & No.classes \\
    \midrule
    Cityscapes\cite{cityscapes} & urban scene & 2048$\times$1024 & 19 \\ 
    DeepGlobe\cite{demir2018deepglobe} & aerial scene & 2448$\times$2448 & 6 \\
    Gleason\cite{gleason2019} & histopathology & 5000$\times$5000 & 4 \\
    \bottomrule
    \end{tabu}
\end{table}

\subsection{Implementation details}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/refinement_module.pdf}
    \caption{{\bf The two residual blocks are trained to refine the segmentation at each scale}. This module outputs the same size $h \times w$ as the input.}
    \label{fig:refinement_module}
\end{figure}

\myheading{Refinement module.} The \Fref{fig:refinement_module} depicts the details of refinement module used in all experiments. The two residual blocks are main parts of this module. With the input of size $h \times w \times 2C$, the refinement module produces the refinement segmentation map of size $h \times w \times C$.

\myheading{Training.} For each dataset, we train a state-of-the-art segmentation model on the whole downsampled images and a refinement module to refine coarse output on sliced patches. The patches are randomly cropped during training the refinement module. During training the refinement module, types of data augmentation are also applied: rotation, and horizontal and vertical flipping. We used SGD optimizer with momentum $0.9$, decayed weight $5\times10^{-4}$ and initial learning rate $10^{-3}$. The refinement module was trained separately in 50 epochs and the learning rate was decreased ten-fold at epoch 20th, 30th, 40th, and 45th. Cross entropy is used as the loss function for training segmentation and refinement modules. We implemented our method using PyTorch \cite{paszke2019pytorch} on top of the public implementation of HRNet-OCR \cite{ocr} and performed training with batch size of 16 on a DGX-1 workstation with Tesla V100 GPU cards. 

\myheading{Testing.} There no overlapping between patches in inference time. The mean intersection over union (mIoU) is used as the evaluation metric for the performance of frameworks. For memory and speed comparison, a machine with CPU Intel Core i7 and a RTX2080Ti card was used for all experiments. 

\subsection{Experiments on the Cistyscapes dataset}
Cityscapes is a dataset of high resolution urban scences, which have the size of $2048\times1024$ pixels, and the task is to segment objects in videos captured by auto cameras. There are two kinds of data, for coarse and fine labeling. In our experiments, we used the fine-labeled dataset, with 2,975 images for training and 500 images for testing.

\subsubsection{Refinement procedure}
The main segmentation network can be any backbone trained with coarse input. This trained network is also reused to produce initial high-resolution segmentation maps. With this dataset, we considered four scale levels ($m=4$), corresponding to patch sizes of $2048\times1024$, $1024\times512$, $512\times256$, and $256\times128$. The size of input image is always $256\times128$ to keep the constant memory usage, so any larger patch size needs to be downsampled. Starting from the coarest segmentation of the size $256\times128$, there are three sequential refinement stages in which the coarse outputs at the previous step are upsampled and refined with high-resolution images. At the end of this post-processing, the coarse segmentation map becomes a fine output with many details.

\subsubsection{Different point selection schemes}
\label{sec:ablation_selection}

\begin{table}[h!]
    \centering
    \caption{{\bf Performance of MagNet on Cityscapes with different schemes to compute query score $\mQ$}. The initial segmentation has the mIoU of $63.23\%$. With $k=0.5 \times h^s \times w^s$, the lin}
    \label{tab:cityscapes__point_strategies}
    \begin{tabu} to \columnwidth {@{}X[1,c]X[1,c]X[1,c]X[1,c]@{}}
    \toprule
    Independent probability & Linear combination & $\alpha$ & mIoU (\%) \\
    \toprule
    \cmark & & - & 66.86 \\
    &\cmark & 1.00 & 67.64 \\
    &\cmark & 0.75 & 67.78 \\
    & \cmark & 0.50 & 68.52 \\
    & \cmark & 0.25 & 66.13 \\
    & \cmark & 0.00 & 66.13 \\
    \bottomrule
    \end{tabu}
\end{table}

The \Fref{tab:cityscapes__point_strategies} illustrates our ablation study about different ways to calculate query score $\mQ$ for picking points to be refined. Overall, the linear combination between certainty and uncertainty scores outperforms the multiplication approach. Moreover, if we use the uncertainty score $\mU$ only ($\alpha=1.0$), the result would be already better than the independent probability approach. 


\subsubsection{Different number of scales}

\begin{table}[h!]
    \centering
    \caption{{\bf Performance of MagNet with and without intermediate refinements on Cityscapes}. It is important to have the intermediate refinements.}
    \label{tab:cityscapes_scales}
    \begin{tabu} to \columnwidth {@{}X[3,l]X[1,c]@{}}
    \toprule
    Refinement steps & mIoU(\%) \\
    \toprule
    256 $\rightarrow$ 2048 & 65.13 \\
    \midrule
    256$\rightarrow$512$\rightarrow$2048 & 67.86 \\
    \midrule
    256$\rightarrow$1024$\rightarrow$2048 & 67.05 \\
    \midrule
    256$\rightarrow$512$\rightarrow$1024$\rightarrow$2048 & 68.52 \\
    \bottomrule
    \end{tabu}
\end{table}

The \Fref{tab:cityscapes_scales} shows the results of our framework on Cityscapes dataset with different number of scales. The intermediate levels yield better improvement due to the reduction in resolution gap between processing stage. While the direct refinement from lowest to highest scale improve

\subsubsection{Accuracy comparison}

The \Tref{tab:cityscapes_result} compares the performance of MagNet with several state-of-the-art semantic segmentation refinment methods. All methods are trained and applied on the output of pretrained HRNetV2-W18 + OCR \cite{ocr} model, which has very competitive results on this dataset. Although the version HRNetV2-W48 + OCR \cite{ocr} can yield higher mIoU, the high complexity of this model makes it inappropriate in terms of memory usage.

In this experiment,  except for DenseCRF \cite{densecrf}, we finetuned other frameworks to achieve the best result with our segmentation backbone. For SegFix \cite{segfix}, with the offset prediction published by the authors, the best result is achieved with the offset width of 10. Both DGF \cite{deepguidedfilter} and PointRend \cite{pointrend} were trained with the output of the segmentation backbone. 

As can be observed, DenseCRF\cite{densecrf} is the only method that cannot improved the coarse segmentation. DGF\cite{deepguidedfilter} improves slightly the mIoU of the initial segmentation model but that is the fastest framework which consumes only 0.2 seconds per image. Having the similar inference time of around 0.

The \Fref{fig:point_comparison} represents the relationship between the accuracy and proportion of points to be refined. The performance of MagNet increases when the proportion of points goes up. The mIoU of this framework reaches the peak at 68.52\% with 50\% points before going down. In contrast, the accuracy of PointRend just increases slightly with small number of refinement points and then the framework has failed to refine the output of coarse segmentation.

\begin{table*}[h!]
    \centering
    \caption{{\bf Performance of MagNet and other semantic segmentation refinement methods in the Cityscapes dataset}. The backbone HRNetV2-W18 + OCR \cite{ocr} is used for all experiment and refinement models are refine outputs of downsampled models.}
    \label{tab:cityscapes_result}
    \begin{tabu} to \textwidth {@{}X[3,l]X[3,l]X[2,l]X[2,l]X[2,l]@{}}
    \toprule
    Segmentation model & Refinement model & mIoU(\%) & Memory(MB) & Inference time (s) \\
    \midrule
    Patch processing & - & 52.19 & 1575 & 1.77 \\
    \midrule
    Downsampling & - & 63.23 & 1575 & 0.02 \\
    \midrule
    Downsampling & DenseCRF\cite{densecrf} & 62.95 ($\downarrow$0.28) & 1575 & 26.02 ($\uparrow$26) \\
    \midrule
    Downsampling & DGF\cite{deepguidedfilter} & 63.33 ($\uparrow$0.10) & 1727 ($\uparrow$152) & 0.22 ($\uparrow$0.2) \\
    \midrule
    Downsampling & PointRend\cite{pointrend} & 64.39 ($\uparrow$1.16) & 2033 ($\uparrow$458) & 0.32 ($\uparrow$0.3) \\
    \midrule
    Downsampling & SegFix\cite{segfix} & 65.83 ($\uparrow$2.60) & 2961 ($\uparrow$1386) & 0.38 ($\uparrow$0.36)\\
    \midrule
    Downsampling & MagNet-Fast & 66.95 ($\uparrow$3.72) & 2007 ($\uparrow$432) & 0.34 ($\uparrow$0.32) \\
    \midrule
    Downsampling & MagNet & 68.52 ($\uparrow$5.29) & 2007 ($\uparrow$432) & 2.93 ($\uparrow$2.91)\\
    \bottomrule
    \end{tabu}
\end{table*}

% \begin{table}[h!]
%     \centering
%     \caption{{\bf Performance of MagNet and other semantic segmentation refinement  methods on the Cityscapes dataset}. In this experiment, we use the same backbone and apply refinement modules on top of the backbone's results}
%     \label{tab:cityscapes_accuracy}
%     \begin{tabu} to \columnwidth {@{}X[3,l]X[2,c]X[2,c]@{}}
%     \toprule
%     Model & mIoU(\%) & Memory(MB) \\
%     \toprule  
    
%     Patch processing & 52.19 & 1575 \\
%     \midrule
%     Downsampling & 63.23 & 1575 \\
%     \midrule
%     Downsampling & \multirow{2}{*}{62.95 ($\downarrow$0.28)} & \multirow{2}{*}{1575} \\
%     + DenseCRF \cite{densecrf} \\
%     \midrule
%     Downsampling & \multirow{2}{*}{63.33 ($\uparrow$0.10)} & \multirow{2}{*}{1727($\uparrow$152)} \\
%     + GuidedFilter \cite{deepguidedfilter} \\
%     \midrule
%     Downsampling & \multirow{2}{*}{64.39 ($\uparrow$1.16)}  & \multirow{2}{*}{2033($\uparrow$458)} \\
%     + PointRend \cite{pointrend} \\
%     \midrule
%     Downsampling & \multirow{2}{*}{65.83 ($\uparrow$2.60)} & \multirow{2}{*}{2973($\uparrow$1368)} \\
%     + SegFix \cite{segfix} \\
%     \midrule
%     Downsampling & \multirow{2}{*}{67.73 ($\uparrow$4.50)} \\
%     + \textbf{MagNet-Lite} \\
%     \midrule
%     Downsampling & \multirow{2}{*}{68.52 ($\uparrow$5.29)} \\
%     + \textbf{MagNet} \\
%     \midrule
%     Downsampling & \multirow{3}{*}{70.10 ($\uparrow$6.87)} \\
%     + \textbf{MagNet} \\
%     + SegFix \cite{segfix} \\
%     \bottomrule
%     \end{tabu}
% \end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/cityscapes_quan_result.pdf}
    \caption{\textbf{Our framework adds more details to the initial segmentation output on Cityscapes dataset}. The frequent mIoU numbers are below the images. More tiny objects are recognized and boundaries are refined better with MagNet and MagNet-Fast (Best viewed in color and zoom).}
    \label{fig:cityscapes_quan}
\end{figure*}

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/point_refinement.pdf}
    \caption{\textbf{Correlation between the proportion of refinement points and mean IoU on the Cityscapes dataset}. When the proportion of refinement points increases, the performance of MagNet continuously grows while the mIoU of PointRend decreases steadily. }
    \label{fig:point_comparison}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/mIoU_distribution.pdf}
    \caption{\textbf{The cumulative distribution of frequent IoU values on Cityscapes dataset (lower is better)}. Both MagNet-Fast and MagNet shift the frequent IoU distribution to the right (Best viewed in color). }
    \label{fig:complexity}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/refinement_step.pdf}
    \caption{\textbf{The cumulative distribution of frequent IoU values on Cityscapes dataset (lower is better)}. Both MagNet-Fast and MagNet shift the frequent IoU distribution to the right (Best viewed in color). }
    \label{fig:complexity}
\end{figure}

\subsubsection{Different backbones}
\begin{table}[h!]
    \centering
    \caption{{\bf Our framework can improve directly the coarse result of different backbones}. The framework trained with HRNet-W32 can refine the output of other models very well.}
    \label{tab:cityscapes_backbones}
    \begin{tabu} to \columnwidth {@{}X[l]X[c]@{}}
    \toprule
    Model & mIoU(\%) \\
    \toprule
    DeepLabv3+ \cite{chen2017deeplab} & 52.01 \\
    \midrule
    DeepLabv3+ \cite{chen2017deeplab} & \multirow{2}{*}{56.60 ($\uparrow$4.59)} \\
    + MagNet \\
    \midrule
    HRNet-W48 + OCR \cite{ocr} & 63.92 \\
    \midrule
    HRNet-W48 + OCR \cite{ocr} & \multirow{2}{*}{54.30} \\
    (Patch processing) \\
    \midrule
    HRNet-W48 + OCR \cite{ocr} & \multirow{2}{*}{68.90 ($\uparrow$4.98)} \\
    + MagNet \\
    \bottomrule
    \end{tabu}
\end{table}

\subsection{Experiments on the DeepGlobe satellite dataset}

\begin{table}[h!]
    \centering
    \caption{{\bf Performance of MagNet and other semantic segmentation methods on the DeepGlobe dataset}. In this experiment, we use the same backbone and apply refinement modules on top of the backbone's results}
    \label{tab:deepglobe_accuracy}
    \begin{tabu} to \columnwidth {@{}X[l]X[c]X[r]@{}}
    \toprule
    Model & mIoU(\%) & Memory (MB) \\
    \toprule
    \textbf{\textit{Downsampling}} \\
    U-net & 50.11 & 1813\\
    FCN-8s & 52.86 & 10569\\
    SegNet & 60.93 & 2645\\
    DeepLabv3+ & 63.50 & 1541\\
    Resnet-FPN & 68.06 & 1105\\
    \midrule
    \textbf{\textit{Patch processing}} \\
    U-net & 46.53 & 1813 \\
    FCN-8s & 62.43 & 10569\\
    SegNet & 68.40 & 2645\\
    DeepLabv3+ & 69.69 & 1541\\
    Resnet-FPN & 70.98 & 1105\\
    \midrule
    GLNet & 71.60  & 1865\\
    \midrule
    MagNet & 72.96  & 1279\\
    \bottomrule
    \end{tabu}
\end{table}

DeepGlobe is a dataset of high resolution satellite images. The dataset contains 803 images, annotated with seven landscape classes. The size of the images is $2048{\times}2048$ pixels. We used the same train/validation/test split as reported in \cite{chen2019collaborative}, with 455, 207 and 142 images for training, validation and testing, respectively. 
\begin{figure}[h!]
	\centering \includegraphics[width=\columnwidth]{figures/deepglobe_result.pdf}
	\caption{\textbf{Our framework performs quality segmentation on DeepGlobe dataset}. The mIoU (numbers below images) at scale 3 is higher than in patch processing and downsampling approaches. While the boundary artifact appears in patch processing due to non-overlapping when sliding, it does not happened in our framework. (Best viewed in color).}
	\label{fig:deepglobe_result}
\end{figure}
\subsubsection{Training procedure}
Our multi-scale segmentation framework can be used with any backbone network, and we chose to use Feature pyramid network (FPN) \cite{seferbekov2018feature} with Resnet-50 \cite{he2016deep} because it was shown to achieve the best performance on this dataset by previous work. We considered three scale levels, corresponding to patch sizes of $2448$, $1224$, and $612$. The size of input image to a segmentation module (i.e., the size that each image patch was rescaled to) was $508$, which was the same as the one used by GLNet \cite{chen2019collaborative}. Other methods were trained and evaluated with publicly available source code from the authors with the same configuration as described above.
%Our framework can work with any backbone, however, Feature pyramid network (FPN) \cite{seferbekov2018feature} with the backbone Resnet-50 \cite{he2016deep} is used due to its highest performance in the previous works on this dataset. The patch sizes respectively are 2448 $\times$ 2448, 1224 $\times$ 1224, and 612 $\times$ 612, those patches are then downsampled to 508 $\times$ 508 like the GLNet \cite{chen2019collaborative}. Other methods are trained and evaluate with the public source code from their authors with the same config as we train MagNet.
\subsubsection{Accuracy comparison}
\Tref{tab:deepglobe_result} compares the performance of MagNet with several state-of-the-art semantic segmentation methods. The methods are grouped into three categories, depending on whether they are downsampling, patch processing, or context aggregation methods.
\begin{table*}[h!]
    \centering
    \caption{{\bf Performance of MagNet and other semantic segmentation methods on the DeepGlobe dataset}. In this experiment, we use squared patches, and the resized patches are also squared. } 
    \label{tab:deepglobe_result}
    \begin{tabu} to \textwidth {@{}X[2,l]X[2.5,r]X[1,r]X[1,r]X[1,r]@{}}
    \toprule
    Model          & Patch width$\rightarrow$Input width & \#patches & mIoU(\%) & Mem.(MB)\\
    \midrule
%    \hfill\\
    % \multicolumn2{l}{\textit{\textbf{Downsampling}}} \\
 %   \midrule
    U-net \cite{ronneberger2015u}   & $2448\rightarrow508$       & 1        & 43.12 & 1813  \\
    FCN-8s \cite{fcn}       & $2448\rightarrow508$       & 1           & 45.62 & 10569  \\
    SegNet \cite{badrinarayanan2017segnet} & $2448\rightarrow508$       & 1           & 52.41 & 2645   \\
    % Resnet-50 FPN  \cite{seferbekov2018feature}  & $2448$       & 1           & 58.60 &  1481\\
    DeepLabv3+ \cite{chen2017deeplab}   & $2448\rightarrow508$       & 1           & 61.30  & 1541  \\
    \midrule
    % \multicolumn2{l}{\textit{\textbf{Patch processing}}} \\
    U-net \cite{ronneberger2015u}   & $612\rightarrow508$ & 16          & 40.55 & 1813 \\
    FCN-8s \cite{fcn}       & $612\rightarrow508$ & 16          & 55.71   & 10569\\
    SegNet \cite{badrinarayanan2017segnet} & $612\rightarrow508$ & 16          & 61.24 & 2645  \\
    DeepLabv3+ \cite{chen2017deeplab}    & $612\rightarrow508$ & 16          & 63.10  & 1541\\
    % Resnet-50 FPN \cite{seferbekov2018feature}   & $612$ & 16          & 66.22 &  1481\\

    \midrule    
    % \multicolumn2{l}{\textit{\textbf{Context aggregation}}} \\
    GLNet \cite{chen2019collaborative} (global)         & $2448\rightarrow508$ & 1          & 62.69   & 1481\\
    GLNet \cite{chen2019collaborative} (local)         &$508\rightarrow508$& 36        & 65.84    & 1395 \\
    GLNet \cite{chen2019collaborative} (aggre.)     & $2448,508\rightarrow 508$  & 1+36          & 65.93    & 1865 \\
    \midrule
    MagNet-1 & $2448\rightarrow508$ & 1           & 58.60   & 1481 \\
    MagNet-2 & $2448,1224\rightarrow508$ & 1+4          & 62.61    & 1407\\
    MagNet-3 & $2448,1224,612\rightarrow508$ & 1+4+16     & \textbf{67.45} & 1369 \\
    \bottomrule
    \end{tabu}
\end{table*}

We trained MagNet for three scales. MagNet-1, MagNet-2, and MagNet-3 refer to the first, second, and third stages of the proposed method, with the patch sizes being $2448, 1224$, and $612$, respectively. That is to increase the strength of the magnifying glass by a factor of four as we move from one stage to the next. 

MagNet-1 corresponds to the coarsest scale, which is  essentially a downsampling method, where the input image is resized to $508$ before it is processed by a segmentation module. The backbone of the segmentation module is ResNet FPN, so the results of MagNet-1 and ResNet FPN are identical in \Tref{tab:deepglobe_result}. MagNet-3 is significantly better than MagNet-2, which is better than \mbox{MagNet-1}. This illustrates the benefits of multi-scale progressive refinement.
 
Compared to MagNet-3, all downsampling methods perform relatively poorly, due to the lossy downsampling operation. MagNet-3 also outperforms patch processing and context aggregation methods. In terms of memory efficiency, MagNet-3 consumes 1481MB GPU memory, which is 25\% lower than the memory required by GLNet \cite{chen2019collaborative}. We used the library 
\textsl{gpustat} to compute the memory usage during the inference time with the batch size of 1.

\Fref{fig:deepglobe_result} shows the segmentation outputs of a downsampling method, a patch processing method, and different processing stages of MagNet. While the patch processing method produces boundary artifact and wrong prediction due to the lack of global context, the downsampling method outputs noisy and coarse segmentation masks. MagNet combines the strengths of both approaches, and it produces a sequence of segmentation masks with increasing quality. 

\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.48\columnwidth}
        \centering
    	\includegraphics[height=0.7\columnwidth,width=\columnwidth]{figures/mIou_distribution.pdf}
    	\caption{Commutative distribution of IoU}
    	\label{fig:deepglobe_worsecase:distribution}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\columnwidth}
        \centering
    	\includegraphics[width=\columnwidth]{figures/deepglobe_worse.pdf}
    	\caption{Examples of decreasing IoU values}
    	\label{fig:deepglobe_worsecase:result}
    \end{subfigure}
	\caption{(a) The commutative distribution of IoU values on DeepGlobe test set (lower is better). There is a right shifting of IoU distribution in the DeepGlobe test set after each scale. (b) Some representative cases when the IoU of one level is lower than the previous one. (Best viewed in color).}
	\label{fig:deepglobe_worsecase}
\end{figure}

\Fref{fig:deepglobe_worsecase:distribution} plots the distribution of IoU values over test images for different processing stages of MagNet. As can be seen, the distribution shifts to the right as MagNet moves from one scale level  to the next. The  mean value increases from around 35\% for MagNet-1 to about 50\% for MagNet-3. 

Overall, in 284 transitions between levels, our framework improved the IoU in 233 (82.04 \%) cases. However, there are 49 cases accounting for 17.25\% in which the IoU decreases from one stage to the next stage. \Fref{fig:deepglobe_worsecase:result} shows some failure cases, where the performance of a processing stage is worse than the performance at the previous stage. This happens when the previous stage misclassifies the majority of a region, and the mistakes are further amplified in the subsequent processing stages.

\subsubsection{Hyper-parameters for consistency loss}
Consistency loss, described in \Sref{sec:regularization}, is an important factor in  our framework. To understand its contribution to the overall performance, we perform several experiments of which the results are shown in \Tref{tab:deepglobe_consistency}. Overall, without using consistency loss (i.e., $\alpha = 0$), the mIoU is 60.93\%. When using consistency loss (i.e., $\alpha = 0.2$) with zero-tolerance margin ($\lambda=0$), the mIoU on the test set increases by 1.2\% to 62.15\%. The mIoU further increases to 62.61\% if the margin value $\lambda$ is set to $0.05$. In all experiments, we used $L_2$ for the consistency loss. We also experimented with $L_1$, but it led to worse performance (mIoU{$=$}61.36\%). We also experimented with having overlapping patches during inference; this increased the processing time but did not yield any performance gain (mIoU{$=$}62.53\%).
\begin{table}[t]
    \centering
    \caption{{\bf Benefits of using consistency loss.} This shows the mIoU values on the test set of DeepGlobe, obtained by different settings of $\lambda$ and $\alpha$ for \mbox{MagNet-2}. The mIoU is significantly lower when the consistency loss is not used ($\alpha=0$)}
    \vskip 0.05in
    \label{tab:deepglobe_consistency}
    \begin{tabu} to \textwidth {@{}X[c]X[c]X[c]@{}}
    \toprule
    $\alpha$ & $\lambda$ & mIoU(\%)\\
    \midrule
    0 &  n/a &       60.93\\
    0.2 & 0 &       62.15\\
    0.2 & 0.05  &   \textbf{62.61}\\
    0.2 & 0.1   &   62.55\\
    \bottomrule
    \end{tabu}
\end{table}


\subsubsection{Different backbones and number of scales}
MagNet can be used with any backbone network. \Tref{tab:deepglobe_backbone} shows the performance of MagNet with three different backbones: U-Net, DeepLabv3+, and ResNet-50 FPN. In all cases, the overall performance indicator, mIoU, increases as we move from one scale level to the next. 

% \begin{table}[h]
%     \vspace{-2.0em}
%     \centering
%     \caption{{\bf Performance of MagNet with different backbones}. In general, any backbone network can be used to obtain a method for progressive refinement with increasing segmentation quality }
%     \label{tab:deepglobe_backbone}
%     \begin{tabu} to \textwidth {@{}X[2,l]X[2.5,r]X[1,r]X[1,c]X[1,r]@{}}
%     \toprule
%     Backbone& Patch width$\rightarrow$Input width & \# patches & mIoU(\%) & Mem.(MB)\\
%     \midrule
%     U-net \cite{ronneberger2015u} & $2448\rightarrow508$ & 1 & 43.12 & 1813\\
%     U-net \cite{ronneberger2015u} & $2448,1224\rightarrow508$ & 1+4 & 47.02  & 1713\\
%     U-net \cite{ronneberger2015u} & $2448,1224,612\rightarrow508$ & 1+4+16 & 47.42  & 1723\\ 
%     \midrule
%     DeepLabv3+ \cite{chen2017deeplab} & $2448\rightarrow508$ & 1 & 61.30  & 1541\\
%     DeepLabv3+ \cite{chen2017deeplab} & $2448,1224\rightarrow508$ & 1+4 & 62.81  & 1441\\
%     DeepLabv3+ \cite{chen2017deeplab} & $2448,1224,612\rightarrow508$ &1+4+16 & 64.49  & 1417\\
%     \midrule
%     Resnet-50 FPN \cite{seferbekov2018feature}&$2448\rightarrow508$ &1 & 58.60  & 1481\\
%     Resnet-50 FPN \cite{seferbekov2018feature} & $2448,1224\rightarrow508$ &1+4& 62.61  & 1407\\
%     Resnet-50 FPN \cite{seferbekov2018feature} & $2448,1224,612\rightarrow508$ &1+4+16&\textbf{67.45} & 1369\\
%     \bottomrule
%     \end{tabu}
% \end{table}


\begin{table}[h]
    \centering
    \caption{{\bf Performance of MagNet with different backbones}. In general, any backbone network can be used to obtain a method for progressive refinement with increasing segmentation quality }
    \label{tab:deepglobe_backbone}
    \begin{tabu} to \textwidth {@{}X[2,l]X[2,c]X[2,c]X[2,c]@{}}
    \toprule
    Backbone& U-net\cite{ronneberger2015u}&DeepLabv3+\cite{chen2017deeplab} & Resnet-50 FPN\cite{seferbekov2018feature}\\
    \midrule
    MagNet-1 & 43.12 & 61.30 & 58.60 \\
    MagNet-2 & 47.02 & 62.81 & 62.61 \\
    MagNet-3 & 47.42 & 64.49 & 67.45 \\
    \bottomrule
    \end{tabu}
\end{table}

\begin{table}[h]
    \centering
    \caption{{\bf Performance of MagNet without and with the intermediate scale  level} (patch width $1224)$. It is important to have the intermediate level to connect the two extreme ends of the scale space }
    \label{tab:deepglobe_level}
    \vskip 0.05in 
    \begin{tabu} to \textwidth {@{}X[3,r]X[2,r]X[2,c]X[2,r]@{}}
    \toprule
    Patch width$\rightarrow$Input width &\# patches & mIoU(\%) & Mem.(MB)\\
    \midrule
    $2448\rightarrow508$ & 1 & 58.60 & 1481\\
    $2448,612\rightarrow508$ & 1+16 & 64.86  & 1355\\
    \midrule
    $2448\rightarrow508$ & 1 & 58.60  & 1481\\
    $2448,1224\rightarrow508$ & 1+4 & 62.61  & 1407\\
    $2448,1224,612\rightarrow508$ & 1+4+16 & \textbf{67.45} & 1369\\
    \bottomrule
    \end{tabu}
\end{table} 

MagNet can also be used with different numbers of scale levels. In the experiments described in this subsection, we have used three scales: $2448 \rightarrow 1224 \rightarrow 612$. We performed an ablation study, where we used only two scales, jumping directly from the coarsest to the finest scales: $2448 \rightarrow 612$. The performance of these two variants are shown in \Tref{tab:deepglobe_level}. In both cases, the mIoU increases as we move from one scale level to the next, and this indicates the robustness of MagNet with the distance between two scale values. On the other hand, the method with three scales is significantly better the method with only two scales. This illustrates the importance of having an intermediate scale connecting the two extreme ends of the scale space, and this justifies the need for our multi-scale segmentation framework. 



 %Overall, our MagNet produces good result on different backbones. After each scale level, the mIoU of any backbone always increases by from 0.4\% to 6\% from previous level. 

 
% Different scale numbers are also tested and the result is showed in the table \Tref{tab:deepglobe_level}. With only 2 scales, the mIoU achieved is around 3\% lower than the same network trained with 3 scales, and 1.5\% lower than the Resnet-50 FPN in the patch processing approach. This problem can be explained by the large margin in resolution between the two scaling levels, which leads to the network at scale 2 believes too much on the prediction produced by the scale 1 module.
% \begin{table}[t]
%     \centering
%     \caption{{\bf Performance on INRIA Aerial dataset}}
%     \label{tab:inria_result}
%     \vskip 0.05in
%     \begin{tabu} to \textwidth {@{}X[l]X[c]X[c]r@{}}
%     \toprule
%     Model          & Patch size & \#patches & mIoU(\%)\\
%     \midrule
%     \textit{\textbf{Downsampling}}\\
%     FCN-8s^{10}    & $5000$   & 1  & 38.65  \\
%     U-net^9 & $5000$   & 1          & 46.58  \\
%     SegNet^{11}  & $5000$   & 1          & 51.87   \\
%     DeepLabv3+^2   & $5000$   & 1      & 52.96    \\
%     \midrule
%     \textit{\textbf{Context aggregation}}\\
%     GLNet^3 (global)    & $5000$  & 1         & 42.50    \\
%     GLNet^3 (local)  & $536$  & 121  & 66.00    \\
%     GLNet^3 (aggregation)     & mixed  & 1+121          & 71.20    \\
%     \midrule
%     MagNet-1 & $5000$ & 1       & 51.68    \\
%     MagNet-2 & $2500$ & 1+4      & 56.36    \\
%     MagNet-3 & $1250$ & 1+4+16       & 68.95 \\
%     MagNet-4 & $625$ & 1+4+16+64      & \textbf{73.40} \\
%     \bottomrule
%     \end{tabu}
%     \vspace{-2.0em}
% \end{table}
\subsection{INRIA Aerial}

\begin{table*}[t]
    \centering
    \caption{{\bf Performance on INRIA Aerial dataset}. In the experiments, we use squared patches and the input images are also squared.}
    \label{tab:inria_result}
    \vskip 0.05in
    \begin{tabu} to \textwidth {@{}X[2,l]X[2,r]X[1,r]X[1,r]@{}}
    \toprule
    Model          & Patch width$\rightarrow$Input width & \#patches & mIoU(\%)\\
    \midrule
    % \multicolumn2{l}{\textit{\textbf{Downsampling}}} \\
    FCN-8s \cite{fcn}    & $5000\rightarrow536$   & 1  & 38.65  \\
    U-net \cite{ronneberger2015u} & $5000\rightarrow536$   & 1          & 46.58  \\
    SegNet \cite{badrinarayanan2017segnet}  & $5000\rightarrow536$   & 1          & 51.87   \\
    DeepLabv3+ \cite{chen2017deeplab}   & $5000\rightarrow536$   & 1      & 52.96    \\
    % \midrule
    % \multicolumn2{l}{\textit{\textbf{Context aggregation}}} \\
    GLNet \cite{chen2019collaborative} (global)    & $5000\rightarrow536$  & 1         & 42.50    \\
    GLNet \cite{chen2019collaborative} (local)  & $536\rightarrow536$  & 121  & 66.00    \\
    GLNet \cite{chen2019collaborative} (aggregation)     & $5000,536\rightarrow536$  & 1+121          & 71.20    \\
    \midrule
    MagNet-1 & $5000\rightarrow536$ & 1       & 51.68    \\
    MagNet-2 & $5000,2500\rightarrow536$ & 1+4      & 56.36    \\
    MagNet-3 & $5000,2500,1250\rightarrow536$ & 1+4+16       & 68.95 \\
    MagNet-4 & $5000,2500,1250,625\rightarrow536$ & 1+4+16+64      & \textbf{73.40} \\
    \bottomrule
    \end{tabu}
\end{table*}
This dataset contains 180 satellite images of resolution $5000$ pixels. Each image is associated with a binary segmentation mask for the building locations in the image. There is class imbalance between the building class and the background class. We trained and evaluated MagNet on this dataset with the same train, validation, and test splits used by GLNet~\cite{chen2019collaborative}, which have 127, 27, and 27 images respectively.
\begin{figure}[h!]
    \vspace{-2em}
	\centering \includegraphics[width=\columnwidth]{figures/inria_result.pdf}
	\caption{Our MagNet outperforms on INRIA Aerial dataset. mIoU (number below images) increases after each stage. (Best viewed in a high-resolution display)}
	\label{fig:inria_result}
\end{figure}


As in the previous subsection, we also used the Feature Pyramid Network~(FPN) ~\cite{seferbekov2018feature} with ResNet-50 \cite{he2016deep} backbone. Because of the larger image size, we extend the framework to have four scale levels with the patch sizes being 5000, 2500, 1250, and 625. For a fair comparison, we assume all segmentation network modules (of MagNet or any other methods) have the same input size of $536$, as used in \cite{chen2019collaborative}. That is to resize an input image or image patch to $536$ pixels before putting through a segmentation module. \Tref{tab:inria_result} shows the mIoUs for various methods. The final output of MagNet, MagNet-4, has mIoU of 73.4\%, which is significantly better than the results obtained by any other method. In particular, MagNet-4 outperforms GLNet \cite{chen2019collaborative}, which is the method that aggregate local and global network branches without any intermediate scales. For MagNet, the mIoU there is a consistent increase between two scale levels. \Fref{fig:inria_result} shows some qualitative results, where the segmentation maps are refined and improved as MagNet analyzes the images at higher and higher resolution.

\subsection{Cityscapes}
Cityscapes is an auto-driving dataset, where images have the size of $2048{\times}1024$ pixels and the task is to segment objects in videos captured by auto cameras. There are two kinds of data, for coarse and fine labeling. In our experiments, we used the fine-labeled dataset, with 2,975 images for training and 500 images for testing. 
% Following the leading method on the leaderboard of the pixel-level semantic segmentation challenge, we used 
We use the popular baseline HRNetV2-W48 \cite{wang2020hrnet} as the backbone network. The size of the input image to this network was set to 1024$\times$512. We trained a MagNet with three scale levels: $2048{\times}1024 \rightarrow 1536{\times}768 \rightarrow 1024{\times}512$. The mIoU of our method comparing with previous ones are shown in \Tref{tab:cityscapes_result}. As can be seen, MagNet-3 yields an mIoU of 78.41 \% which is higher than the origin backbone at the same input size. \Fref{fig:cityscapes_result} shows some segmentation results on the Cityscapes dataset. MagNet-3 refines the segmentation output of MagNet-1, which is the baseline backbone network. 

\begin{table}[h]
    \centering
    \caption{\textbf{Performance on the Cityscapes dataset}. MagNet improves the results from HRNetV2-W48 backbone. In this experiment, the aspect ratio height:width of the original patches and the resized patches is 1:2.}
    \label{tab:cityscapes_result}
    \begin{tabu} to \textwidth {@{}X[3.5,l]X[3,r]X[1,r]X[1,r]@{}}
    \toprule
    Model          & Patch width $\rightarrow$ Input width & \#patches & mIoU(\%)\\
    \midrule
    HRNetV2\cite{wang2020hrnet} (no memory limit) & $2048\rightarrow2048$ &  1 & 79.85  \\
    HRNetV2\cite{wang2020hrnet} & $2048\rightarrow1024$ & 1 &  75.91  \\
    \midrule
    MagNet-1 (i.e., HRNetV2) & $2048\rightarrow1024$ &  1 & 75.91  \\
    MagNet-2 & $2048,1536\rightarrow1024$ & 1+4 &  78.02  \\
    MagNet-3 & $2048,1536,1024\rightarrow1024$ & 1+4+9 & \textbf{78.41}  \\
    \bottomrule
    \end{tabu}
\end{table}

\begin{figure}[t]
	\centering \includegraphics[width=\columnwidth]{figures/cityscapes_res.pdf}
	\caption{\textbf{Segmentation outputs of MagNet-1 (top) and MagNet-3 (bottom) on the Cityscapes dataset}. MagNet-3 yields better qualitative results than MagNet-1 (i.e., HRNetV2-W48 baseline); some small details have been recovered during the iterative refinement process. Best viewed in color.}
	\label{fig:cityscapes_result}
\end{figure}
% \begin{table}[h!]
%     \centering
%     \caption{\textbf{Our MagNet improves the results from HRNet backbones on Cityscapes dataset}}
%     \label{tab:cityscapes_result}
%     \begin{tabu} to \textwidth {@{}X[l]X[c]X[c]r@{}}
%     \toprule
%     Model          & Patch size $\rightarrow$ Input size & \#patches & mIoU(\%)\\
%     \midrule
%     HRNet-W18 & $2048$ &  1 & 76.79  \\
%     HRNet-W48 & $2048$ &  1 & 79.85  \\
%     \midrule
%     {\textit{\textbf{Rescale: $1024$}}} \\
%     HRNet-W18 \cite{wang2020hrnet} & $2048$ & 1 & 73.29   \\
%     MagNet-1 (W18) & $2048$ &  1 & 73.29  \\
%     MagNet-2 (W18) & $1536{\times}768$ & 1+4 &  73.60  \\
%     MagNet-3 (W18) & $1024$ & 1+4+9 & \textbf{73.95}  \\
%     \midrule
%     {\textit{\textbf{Rescale: $1024$}}} \\
%     HRNet-W48 \cite{wang2020hrnet} & $2048$ & 1 &  75.91  \\
%     MagNet-1 (W48) & $2048$ &  1 & 75.91  \\
%     MagNet-2 (W48) & $1536{\times}768$ & 1+4 &  78.02  \\
%     MagNet-3 (W48) & $1024$ & 1+4+9 & \textbf{78.41}  \\
%     \bottomrule
%     \end{tabu}
% \end{table}

% Add examples on Cityscapes dataset
\subsection{Indian Diabetic Retinopathy Image Dataset (IDRID)}
\begin{table}[h!]
    % \vspace{-3em}
    \centering
    \caption{Our MagNet with the VRT U-net backbone yields the best result comparing with downsampling, patch processing or context aggregation method. We use squared patches and rescaled inputs for this experiment.}
    \label{tab:idrid_result}
    \begin{tabu} to \textwidth {@{}X[3,l]X[5,r]X[2,r]X[2,r]@{}}
    \toprule
    Model          & Patch width $\rightarrow$ Input width & \#patches & mIoU(\%)\\
    \midrule
    % \multicolumn2{l}{\textit{\textbf{Downsampling}}} \\
    FCN-8s \cite{fcn}   & $3410\rightarrow640$ & 1  & 14.06  \\
    DeepLabv3+ \cite{chen2017deeplab} & $3410\rightarrow640$ & 1 & 24.66   \\
    SegNet \cite{badrinarayanan2017segnet} & $3410\rightarrow640$ & 1 & 34.84   \\
    VRT U-net & $3410\rightarrow640$ & 1 & 41.64    \\
    % \midrule
    % \multicolumn2{l}{\textit{\textbf{Patch processing}}} \\
    VRT U-net &  $682\rightarrow640$ & 25 & 48.64    \\
    % \midrule
    % \multicolumn2{l}{\textit{\textbf{Context aggregation}}}\\
    GLNet \cite{chen2019collaborative} (global)         & $3410\rightarrow640$  & 1          & 34.56    \\
    GLNet \cite{chen2019collaborative} (local)         & $640\rightarrow640$ & 36  & 41.10    \\
    GLNet \cite{chen2019collaborative} (aggre.)     & $3410,640\rightarrow640$  & 1+36          & 49.17    \\
    \midrule
    MagNet-1 & $3410\rightarrow640$       & 1          & 41.64    \\
    MagNet-2 & $3410,1705\rightarrow640$       & 1+4          & 46.61   \\
    MagNet-3 & $3410,1705,682\rightarrow640$       & 1+4+25          & \textbf{53.28}    \\
    \bottomrule
    \end{tabu}
\end{table}
IDRID is a typical example of medical image datasets, where the images are very large in size, but the regions of interest are tiny. For IDRID, the image size is  $3410$ pixels, and the task is to segment tiny lesions. There are four different types of lesions: microaneurysms (MA), hemorrhages (HE), hard exudates (EX), and soft exudates (SE). We used the EX subset containing 231 training images and 27 testing images. Following the leading method on the leaderboard of the segmentation challenge~\cite{porwal2020idrid}, we used VRT U-Net (see the supplementary material for the network architecture) as the backbone network. The size of the input image to this network was set to $640$. We trained a MagNet with three scale levels: $3410 \rightarrow 1705 \rightarrow 682$. Given the high variation in illumination for fundus images, we applied a data pre-processing step \cite{van2016fast} to unify the image quality and sharpen the texture details. The mIoU of various methods are shown in \Tref{tab:idrid_result}. As can be seen, MagNet yields highest mIoU of 53.28\%.
% \begin{figure}[h]
% 	\centering \includegraphics[width=\columnwidth]{figures/idrid_result.pdf}
% 	\caption{Our MagNet outperforms on IDRID-EX dataset. The lesions has been recognized by the global and refined by the local. The boundary artifact appears in patch processing approach. (Best viewed zoomed in.)}
% 	\label{fig:inria_result}
% \end{figure}
